Representation Matters for Mastering Chess: Improved Feature Representation in AlphaZero Outperforms Switching to Transformers

While transformers have gained recognition as a versatile tool for artificial intelligence (AI), an unexplored challenge arises in the context of chess - a classical AI benchmark. Here, incorporating Vision Transformers (ViTs) into AlphaZero is insufficient for chess mastery, mainly due to ViTs' computational limitations. The attempt to optimize their efficiency by combining MobileNet and NextViT outperformed AlphaZero by about 30 Elo. However, we propose a practical improvement that involves a simple change in the input representation and value loss functions. As a result, we achieve a significant performance boost of up to 180 Elo points beyond what is currently achievable with AlphaZero in chess. In addition to these improvements, our experimental results using the Integrated Gradient technique confirm the effectiveness of the newly introduced features.

==> tables/input_features_v1.tex <==
\begin{table*}[]
\centering
\caption{\small Classical plane representation (version 1) for chess. The features are encoded as a binary maps and features with $\ast$ are single values set over the entire $8\times 8$ plane. The history is represented by a trajectory over the last eight moves.}
%\vspace{.2cm}
\label{tab:inputs_v1}
\begin{tabular}{lccl}
\toprule
%\begin{tabular}{l|c|c|l}
%
\label{tab:input_representation}
\textbf{Feature} & \textbf{Planes} & \textbf{Type}                         & \textbf{Comment}                                                            \\ \midrule
P1 piece                          & 6                                & bool                      & order: \{\texttt{PAWN}, \texttt{KNIGHT}, \texttt{BISHOP}, \texttt{ROOK}, \texttt{QUEEN}, \texttt{KING}\}                                     \\
P2 piece                          & 6                                & bool                      & order: \{\texttt{PAWN}, \texttt{KNIGHT}, \texttt{BISHOP}, \texttt{ROOK}, \texttt{QUEEN}, \texttt{KING}\}                                     \\
Repetitions\textsuperscript{*}                      & 2                                & bool                      & \multicolumn{1}{l}{how often the board positions has occurred} \\
%P1 pocket count\textsuperscript{*}                  & 5                                & \multicolumn{1}{c}{int} & order: \{\texttt{PAWN}, \texttt{KNIGHT}, \texttt{BISHOP}, \texttt{ROOK}, \texttt{QUEEN}\}                                           \\
%P2 pocket count\textsuperscript{*}                  & 5                                & \multicolumn{1}{c}{int} & order: \{\texttt{PAWN}, \texttt{KNIGHT}, \texttt{BISHOP}, \texttt{ROOK}, \texttt{QUEEN}\}                                           \\
%P1 Promoted Pawns                 & 1                                & bool                      & indicates pieces which have been promoted                                    \\
%P2 Promoted Pawns                 & 1                                & bool                      & indicates pieces which have been promoted                                    \\
En-passant square                 & 1                                & bool                      & the square where en-passant capture is possible                        \\
Colour\textsuperscript{*}                           & 1                                & bool                      & all zeros for black and all ones for white                                                   \\
Total move count\textsuperscript{*} & 1 & int & integer value setting the move count (UCI notation)\\
%Total move count\textsuperscript{*}                 & 1                                & int                      & sets the full move count (FEN notation)                                         \\
P1 castling\textsuperscript{*}                      & 2                                & bool                      & binary plane, order: \{\texttt{KING\_SIDE}, \texttt{QUEEN\_SIDE}\}                                      \\
P2 castling\textsuperscript{*}                      & 2                                & bool                      & binary plane, order: \{\texttt{KING\_SIDE}, \texttt{QUEEN\_SIDE}\}                                      \\
No-progress count\textsuperscript{*}                & 1                                & int                      & sets the no progress counter (FEN halfmove clock)                                \\
Last Moves &	16 & bool &	origin and target squares of the last eight moves \\
is960\textsuperscript{*}  &	1 & bool  &	if the 960 variant is active \\
\midrule
Total                             & 39                               &                              &                                                                                           \\
\bottomrule
\end{tabular}
\end{table*}
